Perceptive Locomotion through Whole-Body MPC and Optimal Region Selection

Real-time synthesis of legged locomotion maneuvers in challenging industrial settings is still an open problem, requiring simultaneous determination of footsteps locations several steps ahead while generating whole-body motions close to the robot's limits. State estimation and perception errors impose the practical constraint of fast re-planning motions in a model predictive control (MPC) framework. We first observe that the computational limitation of perceptive locomotion pipelines lies in the combinatorics of contact surface selection. Re-planning contact locations on selected surfaces can be accomplished at MPC frequencies (50-100 Hz). Then, whole-body motion generation typically follows a reference trajectory for the robot base to facilitate convergence. We propose removing this constraint to robustly address unforeseen events such as contact slipping, by leveraging a state-of-the-art whole-body MPC (Croccodyl). Our contributions are integrated into a complete framework for perceptive locomotion, validated under diverse terrain conditions, and demonstrated in challenging trials that push the robot's actuation limits, as well as in the ICRA 2023 quadruped challenge simulation.

==> sections/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/thomas_corberes2.png}}]
	{Thomas Corb\`eres } received his M.Sc. degree in aerospace Engineering engineering from ISAE-SUPAERO Toulouse, France in 2020.
 
 He is currently pursuing a Ph.D. degree in robotics at the University of Edinburgh under the University of S. Tonneau. His research interests include legged locomotion, model predictive control, and contact planning.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/CarlosMastalli.png}}]
	{Carlos Mastalli} received an M.Sc. degree in mechatronics engineering from the Simón Bolívar University, Caracas, Venezuela, in 2013 and a Ph.D. degree in bio-engineering and robotics from the Istituto Italiano di Tecnologia, Genoa, Italy, in 2017.

	He is currently an Assistant Professor at Heriot-Watt University, Edinburgh, U.K.
    He is the Head of the Robot Motor Intelligence (RoMI) Lab affiliated with the National Robotarium and Edinburgh Centre for Robotics.
    He is also appointed as Research Scientist at IHMC, USA.
    Previously, he conducted cutting-edge research in several world-leading labs: Istituto Italiano di Tecnologia (Italy), LAAS-CNRS (France), ETH Zürich (Switzerland), and the University of Edinburgh (UK).
    His research focuses on building athletic intelligence for robots with legs and arms.
    Carlos' research work is at the intersection of model predictive control, numerical optimization, machine learning, and robot co-design.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/wolfgang.jpg}}]
{Wolfgang Merkt} received the B.Eng.(Hns) degree in mechanical engineering with management and the M.Sc.(R) and Ph.D. degrees in robotics and autonomous systems from the University of Edinburgh, Edinburgh, U.K., in 2014, 2015 and 2019, respectively.

He is currently a Postdoctoral Researcher at the Oxford Robotics Institute, University of Oxford. During his Ph.D., he worked on trajectory optimization and warm starting optimal control for high-dimensional systems and humanoid robots under the supervision of S. Vijayakumar. His research interests include fast optimization-based methods for planning and control, loco-manipulation, and legged robots.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Ioannis.Havoutis.2019.jpg}}]
{Ioannis Havoutis} received the M.Sc. in artificial intelligence and Ph.D. in Informatics degrees from the University of Edinburgh, Edinburgh, U.K. He is a Lecturer in Robotics at the University of Oxford.

He is part of the Oxford Robotics Institute and a co-lead of the Dynamic Robot Systems group. His focus is on approaches for dynamic whole-body motion planning and control for legged robots in challenging domains. From 2015 to 2017, he was a postdoc at the Robot Learning and Interaction Group, at the Idiap Research Institute. Previously, from 2011 to 2015, he was a senior postdoc at the Dynamic Legged System lab the Istituto Italiano di Tecnologia.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/jshim.jpg}}]
{Jaehyun Shim}  received a B.Eng. degree in mechanical engineering from the University of Tokyo, Tokyo, Japan in 2015 and an M.A.Sc. degree in mechanical engineering from the University of British Columbia, Vancouver, BC, Canada, in 2018.
He is currently a Software Engineer at the University of Edinburgh. He worked on developing autonomous delivery robots as a Software Engineer at ROBOTIS, Seoul, South Korea. His research interests include optimization-based planning and legged robots.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/maurice_fallon.jpg}}]
{Maurice Fallon} studied Electronic Engineering at University College Dublin. His Ph.D. research in the field of acoustic source tracking was carried out in the Engineering Department of the University of Cambridge.

After his Ph.D. he moved to MIT as a post doctoral researcher and later research scientist in the Marine Robotics Group (2008-2012). From
2012-2015 he was the perception lead of MIT’s team in the DARPA Robotics Challenge. From 2015, he was a Lecturer at University of Edinburgh where he led research in collaboration with NASA’s humanoid robotics program. He moved to Oxford in April 2017 and took up the Royal Society University Research Fellowship in October 2017.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/nicolas_mansard.png}}]
{Nicolas Mansard} is CNRS researcher (“charg\'e de recherche CNRS”) since 2009. He received the M.Sc. in computer science of Univ. Grenoble in
2003 and the PhD in robotics of Univ. Rennes in 2006.

He was then post-doctoral researcher in Stanford Univ. with O. Khatib in 2007 and in
JRL-Japan with A. Kheddar in 2008. He was invited researcher in Univ. Washington with E.Todorov in 2014. He received the CNRS Bronze Medal in 2015 (one medal is award in France in automatic/robotic/signal-processing every year). His main research interests include the motion generation, planning and control of complex robots, with a special regard in humanoid robotics. His expertise covers sensor-based (vision and force) control, numerical mathematics for control, bipedal locomotion and locomotion planning. He published more than 70 papers in international journals and conferences and supervised 10 PhD thesis. He is currently associate editor of IEEE Transactions on Robotics.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/thomas_flayols.jpeg}}]
{Thomas Flayols} is a contract researcher at LAAS-CNRS in the Gepetto group, where the graduated from his PhD in 2018. Before that he graduated from Ecole Normale Supérieure de Cachan (ENS) with a Master Degree in Embedded Systems and Industrial Computing.

His research interest focuses on force control of legged robots for locomotion and stabilization. He has a particular interest in experimental validation of estimation and control techniques. He is also a mechatronic engineer attached to open hardware design applied to actuation and perception for robotic.
Currently, he is actively contributing to the design of the open source quadruped robot ODRI initiated by the MPI of Tübingen.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Sethu2019.jpg}}]
{Sethu Vijayakumar} received the Ph.D. degree in computer science and engineering from the Tokyo Institute of Technology, Tokyo, Japan, in 1998.

He is Professor of Robotics and a Director with the Institute of Perception, Action, and Behaviour, School of Informatics, University of Edinburgh, U.K., where he holds the Royal Academy of Engineering Microsoft Research Chair in Learning Robotics. He also has additional appointments as
an Adjunct Faculty with the University of Southern California, Los Angeles, CA, USA and a Visiting Research Scientist with the RIKEN Brain Science Institute, Tokyo. His research interests include statistical machine learning, robotics, planning and optimization in autonomous systems to human motor control, and optimality. Dr. Vijayakumar is a Fellow of the Royal Society of Edinburgh.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[draft=false, width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/steve_tonneau.png}}]
{Steve Tonneau} received the Ph.D. degree in humanoid robotics from the INRIA/IRISA, France, in 2015.

He is a Lecturer at the University of Edinburgh, Edinburgh, U.K.. Previously, he was a Postdoctoral Researcher at LAAS-CNRS in Toulouse, France. His research focuses on motion planning based on the biomechanical analysis of motion invariants. Applications include computer graphics animation as well as robotics.
\end{IEEEbiography}


==> sections/old_introduction.tex <==


\section{Introduction}

% \stn{
%     What is the problem? Why is it interesting and important} \\
    
Developing reliable and autonomous locomotion for legged robots in arbitrary environments is a longstanding challenge. An ideal motion synthesis framework would automatically execute motions that satisfy a task roughly specified by a non-expert.
The hardware maturity of quadruped robots~\cite{ANYmal-robot,unitree-robot,Spot-robot,ghostrobotics-robot} motivates the development of such a framework for industrial applications including inspections in hazardous environments or industrial areas~\cite{ARGOS}. These objectives highlight the need for improving robot capabilities and reliability from an algorithmic point of view. We focus on locomotion, from local detection of the environment to motion generation, commonly referred to as \textbf{perceptive locomotion}. A  robust footstep planning, environment detection and control is essential for perceptive locomotion, especially for legged robots, where contact interactions introduce estimation errors. The integration of these components, each the topic of active research, is a technological and scientific challenge. 
%We are interested in understanding how to link these components together in the context of dynamic multi-contact locomotion.



Blind \textbf{controllers} have demonstrated capabilities to adapt and maneuver in challenging terrain using only proprioceptive information~\cite{Bledt-cheetah3-design, Gehring-dynamic-trotting-slopes, Gehring-agile-motions-quadruped, focchi2019heuristicplanning}. With reinforcement learning methods, it is possible to synthesise controllers that are robust to various types of environments~\cite{Hwango-learning-motor-skills-ANYmal,2017-TOG-deepLoco,Xie-Dynamic-randomization-quadruped}, including stairs~\cite{Siekmann-Cassie-blind-bipedal-stairs} or in the wild~\cite{Lee-learning-hallenging-terrain-ANYmal}. Still, these methods need to be complemented with exteroceptive perception as it is otherwise impossible to detect gaps and holes in the environment.

% This paper is a technical synthesis\stn{ca limite un peu la contribution} of \std{many} different works \stn{lesquels} and propose a complete pipeline from detection to motion generation in clustered environment. 
%Adaptation to complex scenarios requires a generic method and yet computational still efficient to allow real-time application. 
In such cases a problem of discrete \textbf{combinatorics} arises, where a choice must be made between multiple surfaces  to step on~\cite{Tsounis-DeepGait,Fernbach-CROC,Tonneau-Acyclic-planner,Fankhauser2018ProbabilisticTerrainMapping}. This additional decision layer must be reliable to ensure feasible motions while being compatible with real-time applications.
To ensure stability, trajectory tracking and reactivity, the whole-body \textbf{controller} needs to be robust to external perturbations. Navigating in a non-trivial environment. Our research question is thus to determine how to link these components to allow for reliable and reactive planning and control. 

% This synthesis aims to find a trade-off between different methods to generate complex motion while staying relatively simple and computationally efficient. 
% \stn{Ici c est le paragphra clef. Il faut essayer un peu de developer sur: quels sont les questions / enjeux que posent l integration, et quelles sont les hypotheses qui sont faites , un peu comme sur le papier iros} 

\begingroup
\def\boxit#1#2{%
  \smash{\llap{\rlap{\hspace{4pt}\href{#1}{\strut\raisebox{\height}{\phantom{\rule{0.98\linewidth}{#2}}} } }~}}\ignorespaces}
% No borders around the hyperlink areas
\hypersetup{pdfborder=0 0 0}
\begin{figure}[t]
    \boxit{\videoLink{135}}{95pt}%
    \includegraphics[trim ={0px 50px 350px 00px}, clip,width =\linewidth, keepaspectratio = true]{figures/intro/walk_down_stairs.png}
    \vspace{-5mm}
    % \includegraphics[trim ={0px 50px 350px 00px}, draft=false clip,width =\linewidth, keepaspectratio = true]{figures/intro/walk_down_stairs.png}
    \caption{Industrial staircase descent with on-board perception. Video: 
    \videoLink[0]}
    \label{fig::intro_walk_down}
\end{figure}
\endgroup

% \stn{Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? }

% \stn{avant de developper ici, le paragphe du haut aurait du lever autant de problemes que de paragraphes qui suivent. Et ensuite ici en gras tu peux les reprenedre, par exemple \stn{control:}}


%To deal with the \textbf{combinatorics} of contact planning, simplified models are usually incorporated within an extra decision layer, where a terrain representation is used to evaluate where the next footsteps should occur~\cite{Tsounis-DeepGait,Fernbach-CROC,Tonneau-Acyclic-planner,Fankhauser2018ProbabilisticTerrainMapping}.

Our method belongs to the family of hierarchical approaches where, both for computational performance and convergence issues, it is common to first fix compute contact positions and then whole-body motions~\cite{escande:hal-00751924,Deits2014FootstepPO,Ponton_2021}. We propose to relax the footstep constraints by only selecting the convex surfaces obtained in the planning phase. In addition, we propose to adapt footstep positions and motions to the environment. This is achieved through the introduction of a dedicated QP-based optimisation routine between the contact planner and whole-body controller. This approach has proven beneficial in our previous work~\cite{risbourg:hal-03594629} on the Solo robot. This benefit is demonstrated further here on the ANYmal B robot with a novel whole-body model-predictive controller (MPC)~\cite{Agile-Maneuvers-mastalli}. The MPC is based on the robot's full dynamics, which allow joint-torque constraints. Our design choices aim at fully leveraging this capability by letting the MPC determine body posture without constraining it. This is essential in complex environments where torque limits may be reached. Additionally, we propose a complete method to detect the environment with an external depth-camera sensor and extract convex planes suitable for planning motions with mixed-integer programs.

% \std{Two similar approaches to ours, especially in terms of architecture of control with a decoupling between body generation and foostep planning, have been recently proposed and tested on ANYmal-C. In~\cite{Jenelten_2022_TAMOLS}, a chain of filtering of the heightmap is used to optimize the footstep position, the torso orientation and obstacle avoidance for the foot trajectory. A more condensed architecture has been proposed by~\cite{Grandia-perceptive-through-NMPC} with a non-linear MPC that can simultaneously plan the obstacle-free trajectory of the end-effector trajectory and the body. Yet important differences remains in the planning stage adopted for the surface contact selection and on the motion generation strategies.} \stn{which are? I d maybe just say that the approaches are complementary as discussed in section. If we talk about these papers later actually just remove them from the intro}

% \tc{old version}

% Including the perception of the environment brings up the question of the choice of contacts and the need to take these \textbf{combinatorics} into account. With a local height-map of the environment surrounding the robot, in \cite{Tsounis-DeepGait} a hierarchical architecture is introduced to overcome wide gaps in simulation and adapt the gait pattern as well with a higher level gait generator. The gait and foothold planner is based on a convex simplification of the dynamic of the centre of mass (CoM)~\cite{Fernbach-CROC} for stable transitions between contacts which results in conservative motions. A similar approach is presented in~\cite{Gangapurwala-RLOC} with a complete pipeline tested on ANYmal-C robot with a higher level of footstep position selection. Another work presented in~\cite{Fankhauser-Robust-rough-ETH} proposes a robust pipeline for selecting footsteps based on statically stable gait criteria and sampling-based search.  
% % While these approaches allow impressive terrain adaptation, the locomotion remains non-agile.
% Our method belongs to the family of hierarchical approaches where a high-level decision deals with the combinatorics. 


% % \stn{
% % )
% %     What are the key components of my approach and results? Also include any specific limitations. }

% \stn{maybe the comparison with other works can be skipped here for related works, or at least compressed.}
% The salient aspects of our locomotion framework are a mixed-integer program to tackle the combinatorics of contact surface selection and a whole-body model predictive controller (MPC) to generate the robot's full-body motion. With the term whole-body, in our perspective, we refer to a MPC based on the full dynamics of the robot and enabling especially to penalise the torques. We have chosen a decoupled approach where we only use the first contact surface of the high-level decision plan, and continuously re-adjust the trajectory of the feet to adapt to disturbances and avoid obstacles. It aims to find a balance between following a reliable plan and letting the whole-body MPC make more decisions about adjusting the body posture. Recently, two approaches similar to ours have been proposed for ANYmal C. In~\cite{Jenelten_2022_TAMOLS}, a chain of filtering of the heightmap is used to optimize the footstep position, the torso orientation and obstacle avoidance for the foot trajectory. An architecture more condensed has been proposed by~\cite{Grandia-perceptive-through-NMPC} with a non-linear MPC that can simultaneously plan the obstacle-free trajectory of the end-effector trajectory and the body. However, there are still significant differences in the design architecture. Both solutions require an additional layer to plan the torso motion. As an alternative, we let the MPC generate the torso's motion that allows the robot to cross more challenging obstacles and as its own pace. We make use of the full capabilities of the whole-body dynamic model by using a Ricatti-gain controller to follow the flow of the optimal control problem (OCP) without relying on an additional instantaneous whole-body controller. As a last difference, our approach uses mixed-integer programming to choose the contact surface, ensuring the reliability of the contact plans. 


%\subsection{Contribution}

Our key contributions are:
\begin{itemize}
    \item An open-source and generic method for legged robots to cross challenging terrain.
    \item A perceptive locomotion framework that extracts convex planes for planning footstep plans using mixed-integer programs. 
    \item A method to effectively integrate a high-level contact planner with a whole-body MPC that reactively updates foot positions and trajectories.
    \item A thorough validation of the pipeline over a wide range of experimental trials, to understand the potential and limits of our approach.
\end{itemize}

==> sections/sota.tex <==
\section{Related Work}


\subsection{Multi-contact locomotion}
\label{sec::multi-contact-sota}

Multi-contact locomotion planning involves determining the robot's motions, contact surfaces and timings to step on, which is often computed in a decoupled fashion. To do so, different approaches have been studied and can be categorized into two groups: \textit{all-at-once approaches} where we seek to optimise all parameters at the same time and \textit{decomposed approaches} in which the problem is divided into sub-problems easier to solve, usually for computing time efficiency.

\subsubsection{All-at-once approaches}
This approach can be treated as a large non-linear problem in which all decision variables are optimised at the same time. This can include contact timings, contact surfaces, CoM and whole-body motions. Due to this, more potential contact modes may be discovered than pre-specified contact schedule. In \cite{Mordatch2012DiscoveryOC}, an additional variable indicates whether the body is in contact and modifies the contact invariant cost and dynamics. Another way to formulate multi-contact dynamics is to rely on complementary constraints \cite{Posa-TO-contact} to avoid prior reasoning about contact timing or contact selection. In \cite{Cleac-Contact-implicit-MPC}, a MPC is formulated as a bi-level optimisation which uses the derivatives of the contact implicit dynamics expressed as a linear complementarity problem. Despite the fact that this approach relies on offline calculations and the planning horizon is short, it can adapt the contact sequence online to face disturbances. Complementarity constraints allow abstracting the contact modes. However, optimising these mode-invariant trajectories usually requires a smooth dynamic contact model to retrieve useful information around the contacts, which is achieved via contact smoothing. In this context, \cite{Pang-global-contact-rich} proposes a convex and differentiable contact dynamic model combined with a sampling-based planner to efficiently discover new contact behaviours in manipulation scenarios. Similarly, \cite{Lidec-leveraging-RS-OC} introduces randomized smoothing techniques to get more exploratory behaviour since local gradient information is poor with such contact dynamics. 

% \stn{je pense doit aussi y avoir un posa plus recent et un papier de manchester. Aussi 2 papiers de justin Augmenting differentiable physics with randomized smoothing  et Leveraging Randomized Smoothing for Optimal Control of Nonsmooth Dynamical Systems. Enfin un recent de tedrake Global Planning for Contact-Rich Manipulation via Local Smoothing of Quasi-dynamic Contact Models}\tc{posa plus recent ? Real-Time Multi-Contact Model Predictive Control via ADMM ? manchester : ok justin : ok ( c'est pas les 2 memes les papiers que tu a cite ? tedrake : ok}. 

In a similar fashion, TOWR \cite{winkler18} generates highly dynamic trajectories by solving a large non-linear problem while abstracting the contact modes. Some drawbacks, however, prevent its practical use in real robots, e.g., computation time, feasibility of optimized motion and need for good initialisation. In recent years, efforts have been made to improve TOWR for real application. In \cite{Melon-TOWR-Learning}, a whole-body controller adapts optimised motions into feasible trajectories for the ANYmal robot. Additionally, data-driven initialisationimproves TOWR's computation timing and success rate. Moreover, \cite{Melon-towr-receiding} proposes a perceptive pipeline that allows re-planning motions at \SI{1}{\hertz}. 
% Although this approach may appear more complete, the resulting motions on the hardware remains non agile. \stn{as opposed to what? Maybe simply remove that last sentence. } 



\subsubsection{Decoupled approaches}
\label{sec:decoupled-approaches}
We can decompose the problem into smaller sub-problems that can be solved faster. This is achieved at the cost of using reduced models or assumptions that produce conservative motions. In order to generate complex and dynamic behaviours while keeping the computation time low, we must find the most appropriate trade-off. Another key challenge is the integration of these different sub-problems. Most successful real-time approaches follow this approach. Impressive perceptive pipelines on the LittleDog robot have been proposed \cite{Zucker-Optimisation-LittleDog, Kolter-LittleDog, Kalakrishnan-LittleDog} and have inspired further works \cite{Fankhauser-Robust-rough-ETH}. However, they all require high-precision terrain pre-mapping and an external motion capture system. 

Decomposing the problem does not allow us to avoid solving the combinatorial problem even with a simpler or more conservative model when dealing with multi-contact scenarios. One way is to use sampling-based methods with efficient heuristics and constraints to select contact surfaces~\cite{Tonneau-Acyclic-planner, Fankhauser-Robust-rough-ETH, Zucker-Optimisation-LittleDog}. Another one is to formulate this problem as a mixed-integer formulation (e.g, \cite{Deits2014FootstepPO, aceituno_cabezas-ral18, tonneau:sl1m:9454381}) which can be more efficient when dealing with convex problems. At the cost of higher computing time, especially in worst-case scenarios, these formulations find the optimal solution for the cost function given.


It is common to optimise the end-effector trajectory in a sub-problem to reduce the complexity of handling collision avoidance in the whole-body planning process. The complete gradient-based optimiser proposed in \cite{Ratliff-CHOMP} generates smooth trajectory planning for robotic arms or legs. The LittleDog robot~\cite{Zucker-Optimisation-LittleDog} to account for knee collision. One of the drawbacks is the computing time, around \SI{50}{\milli\second} as mentioned in \cite{Kalakrishnan-LittleDog}, which penalises more reactive applications. Other methods focus on the end-effector trajectory~\cite{Fankhauser-Robust-rough-ETH} by modifying the way-points of a cubic hermic spline depending on the terrain. Regarding only the end-effector trajectory, more precise techniques allow to optimise the time spent in each area of the environment as proposed for a UAV trajectory with a bi-level optimisation in \cite{Sun-UAV-bilevel}. The problem could also be formulated as a mixed-integer optimisation to select the relevant area of the space to cross \cite{Deits2015EfficientMP} but the constraint on computation time motivates a more conservative formulation.


\subsection{Model of the dynamics}
% \stn{y a vraiment bcp sur la dynamique. Ca me surprend sur un papier integratif. Mais d un autre cote ça semble pertinent. A voir ce que dit thomas flayols  }

Due to computational challenges, many works employ simplified dynamic models to avoid high non-linearity. We describe dynamic models commonly used in model-based control techniques in this section, and how they are typically used starting from abstract representations. We refer to \cite{Wensing-review-opimisation-based} for a more general study.

A first model that emerged for humanoid robots and developed later for quadruped locomotion is the linear inverted pendulum (LIP) model \cite{Kajita-LIP} when linearizing the unactuated part of the dynamics by considering a constant height and no angular momentum around the center of mass on flat ground. This allows controlling the CoM by constraining the zero-momentum point (ZMP) to lie inside the convex hull of the contact points \cite{Kajita-ZMP}. This model has been studied and improved for multi-contact scenarios \cite{Caron-ZMP-multicontact}, or to mitigate the assumptions by including actuation limits \cite{Orsolino-Wrench-based}.
 
Another common assumption for quadruped locomotion is the Single Rigid Body model (SRB) \cite{Cheetah3-convex,winkler18}. Considering the legs are massless (i.e., the trunk's rotational inertia is constant) allows us to plan the motion directly by optimising the contact forces and CoM. Consequently, a two-stage architecture is possible~\cite{leziart:hal-03052451,Kim-WBIC}, where the MPC plans CoM trajectories and contact forces, while the whole-body controller track the latter. This model allows stabilizing highly-dynamic gaits, and including extra decision variables such as footstep positions~\cite{Bledt-Heuristics}.

These reduced models are included in more general centroidal dynamics, in which dynamics are reduced to their unactuated parts. This implies that there is enough torque power to execute the motion \cite{Dai-centroidal-atlas}. This model remains non-linear but convex approximations are possible~\cite{Ponton_2021,Fernbach-CROC}. 

These different models require a whole-body controller to instantaneously track the control quantities and ensure closed-loop stability by computing the desired torques or joint velocities. Two main controllers have been developed: first a hierarchical least-square optimisation where the lower task is optimised inside the null space of the higher task to ensure a strict hierarchy between the objectives~\cite{escande:hal-00751924}; second, a weighted Quadratic Programming and assign the weights depending on the task priority~\cite{Kim-WBIC}. 

However, the feasibility of the plan proposed by the reduced model is not guaranteed, and its execution may conflict with the stability tasks proposed in the lower controller. Even though some works has focused on establishing properly a consensus between them \cite{Herzog-kino-dynamic-motion,Budhiraja-consensus-dyn}, using a whole-body dynamic model is promising to overcome these challenges. More recently, thanks to the progress of numerical optimisation tools for OCPs \cite{crocoddyl20icra,Andersson2019-casadi,carpentier2018analytical}, considering the whole-body dynamics inside the optimal control problem (OCP) has been made possible \cite{Agile-Maneuvers-mastalli,assirelli:hal-03778738,Neunert-NMPC,Katayama-inverse-dyn-mpc}. Contrary to the previous methods, this allows to formulate a state feedback controller that does not compete with the OCP \tc{that optimises the motion}\stn{with what ocp?}. However, it usually requires good initial guess and the horizon is restricted around 1 or 2s due to the higher computing time, which prevents reasoning and planning motions over a longer period of time, as opposed to reduced models.


\subsection{Perception}

Including information of the surroundings in the decision-making process is necessary to increase the capabilities and cross challenging terrain such as gaps, holes or steps. The environment is typically modelled as an elevation map by fusing depth sensor information within proprioceptive information\cite{Fankhauser2018ProbabilisticTerrainMapping}. \cite{Miki-ANYmal-wild-perception} have proposed a robust way of combining both pieces of information, which allows ANYmal-C robot to navigate along hiking trails. \tc{Recently, in~\cite{Jenelten_2022_TAMOLS}, a interesting chain of filtering of the heightmap is used to optimize the footstep position, the torso orientation and obstacle avoidance for the foot trajectory}. Processing the elevation map by attributing a cost for safe foothold placement allows to plan safely the footstep with sampling based methods \cite{Fankhauser-Robust-rough-ETH, Mastalli-onboard-perception}. An alternative way of representing the environment is to extract a set of surfaces in order to handle the combinatorics with mixed-integer optimisation \cite{Deits2014FootstepPO}. In \cite{Grandia-multi-layer-CBF}, a low frequency MPC with a reduced model of the dynamic optimises the contact location within a safe convex region by using a control barrier function to ensure the stability in closed loop of the system. The convex surface choice relies on a heuristic that selects the closest surface when the landing effector is in the middle of the flying phase. In \cite{Grandia-perceptive-through-NMPC}, the authors take advantage of both formulations. The convex representation helps assigning the next contact location and impose inequalities in the optimal control formulation whereas the heightmap is used to handle collision avoidance constraints. Our approach relies on a convex representation of the environment but allows to use additional information from the height map environment for the obstacle avoidance as described later in Sec.~\ref{sec::collision-free-traj}. A more recent approach is to map the visual inputs to high-level decision actions \cite{Margolis-learning-pixel}, or to directly map visual inputs along with proprioceptive information to joint position command \cite{Imai-Vision-Guided}. This methods seems more relevant when the explicit state representation is not required as it is the case with reinforcement learning method. 



